On Star operation and some ideals on the Baire space

We investigate several $\sigma$-ideals on the Baire space $\omega^\omega$ $(\mathbb{Z}^\omega)$, introducing and studying the ideals $\mathcal{G}$ and $\mathcal{SMZ}^+$, alongside the classical ideals of meager sets, strong measure zero sets, the eventually different ideal and infinitely equal ideal We establish structural relationships and proper inclusions among these ideals. Also we compute the cardinal invariants of $\mathcal{M}_-$, proving that they are same as invariants of $\sigma$-ideal of meager sets. We further analyze the operation $^*$ on families of sets, establishing dual relationships such as $\mathcal{ED}^* = \mathcal{IE}$, $\mathcal{IE}^*=\mathcal{ED}$, $\mathcal{M}_-^*=\mathcal{SMZ}^+$ and $\mathcal{H}^* = \mathcal{G}$, and derive separations between ideals under additional set-theoretic assumptions. Finally, we prove a tree dichotomy theorem for the ideal $\mathcal{M}_-$ and we study the associated forcing notion.

==> 1_rozdzial_orginal.tex <==
In this chapter, we will introduce some new ideals $\mathcal{G}$ and $ \mathcal{SMZ}^+$ in the Baire space. We will investigate the structural relationships and interactions between these ideals and other known ideals in the Baire space.


We will begin by recalling the characterization of meager sets in the Cantor space often referred to as 'chopped reals'.
\begin{df}
    For $x\in 2^\omega $ and $\bar{I}\in \mathbb{IP}$ define 
    \begin{center}
        $F(x,\bar{I})=\{y\in 2^{\omega}: \forall^{\infty} n \;\;    x\upharpoonright I_n\neq y\upharpoonright I_n\}$
    \end{center}
\end{df}
The following theorem gathers basic properties of chopped reals.
\begin{thm}(Talagrand; \cite{BBB}, see also Bartoszyński and Judah; \cite{BBB})\label{XD}

    \begin{itemize}
    \item [--] For every $x\in 2^\omega$ and $\bar{I}\in \mathbb{IP} $ set $F(x,\bar{I})$ is meager,
    \item    [--] for every meager set $F\subseteq\Cantor$ we have $F\subseteq F(x,\bar{I})$ for some $x\in 2^\omega$ and interval partition $\bar{I}$,

        \item  [--] if $I\sqsubseteq^* J$ then $F(x,\bar{I})\subseteq F(x,\bar{J}),$
        \item [--] if    $F(y,\bar{I})\subseteq F(z,\bar{J})$, then $  \bar{I}\sqsubseteq^*\bar{J},$
        \item [--] $F(x,\bar{I})+y=F(x+y,\bar{I})$.
    \end{itemize}
\end{thm}
 Strong measure zero sets were defined originally on the real line, by Borel, but we can translate the definition   from $\mathbb{R}$ to $2^\omega$.


\begin{df}
    A set $A \subseteq 2^\omega$ has strong zero measure $(A\in \mathcal{SMZ})$ if for every sequence $(k_n)_{n<\omega}$ of natural numbers there exists a sequence $(\sigma_n)_{n<\omega}$ such that  $A\subseteq \bigcup_n [\sigma_n]$ and $|\sigma_n|=k_n$  for every $n<\omega$.
\end{df}

Next, we move to the characterization of strong measure zero sets in the Cantor space.

\begin{thm}(Bartoszyński, Judah; \cite{BBB})\label{xdxdxd}
 Set $X\subseteq2^\omega$ has strong measure zero if and only if for every interval partition $\bar{I}\in \mathbb{IP}$ there exists $z\in 2^\omega$ such that:
 $$\forall x\in X\;\; \exists^\infty n\;\; x\upharpoonright I_n=z\upharpoonright I_n.$$
\end{thm} 

The relationship between strong measure zero sets and meager sets on the real line was first shown in \cite{galvin1973strong} by Galvin, Mycielski, and Solovay. Alternatively, this connection can be proven by using the  characterizations of these two ideals.

\begin{thm}(Galvin, Mycielski, Solovay; \cite{galvin1973strong})
    $X\in\mathcal{SMZ}$ iff and only iff for all $H\in \mathcal{M}$  we have $X+H\neq 2^\omega$.
\end{thm}



In  \cite{Wohofsky}, Wohofsky showed that the Galvin-Mycielski-Solovay Theorem doesn't hold in the Baire space $(\mathbb{Z^\omega})$. He showed that $\mathcal{M}^*\subseteq\mathcal{SMZ}$, and that assuming the Continuum Hypothesis it is possible to construct a  set $X\in \mathcal{SMZ}\backslash \mathcal{M}^*.$ 

The characterization of meager sets was adapted to the Baire space in \cite{EEEE}. However, it turns out that in the Baire space, this is not characterization of meager sets. 


\begin{df}
%    A set $X\in \omega^\omega $ (or $\mathbb{Z}^\omega $) is $\mathcal{M}_-$ if $X\subseteq M(x,I)$ for some interval partition $I$ and $x\in \mathbb{Z}^\omega$.

Let $\mathcal{M}_-$ be a $\sigma$-ideal generated by the sets 
\begin{center}
$M(x,\bar{I})= \{y\in \mathbb{Z}^{\omega}: \forall^{\infty} n \;\;    x\upharpoonright I_n\neq y\upharpoonright I_n\}$  
\end{center}
for $x\in \mathbb{Z}^\omega$ and $\bar{I}\in \mathbb{IP}.$
\end{df}

All the properties from \ref{XD} holds for sets from $\mathcal{M}_-$ ideal.

Now we will rewrite definition and characterizations of  strong measure zero sets to the Baire space. 

\begin{df}
    A set $A \subseteq \mathbb{Z}^\omega$ has strong zero measure $(A\in \mathcal{SMZ})$ if for every sequence $(k_n)_{n<\omega}$ of natural numbers there exists a sequence $(\sigma_n)_{n<\omega}$ such that  $A\subseteq \bigcup [\sigma_n]$ and $|\sigma_n|=k_n$  for every $n<\omega$.
\end{df}

The same argument as the one for Cantor space can be used to prove the following result.

\begin{proposition}
    A set $X\subseteq \mathbb{Z}^\omega$ has strong measure zero if and only if for every increasing sequence $k_n\in \omega^\omega$ there exists $(\sigma_n)_{n<\omega}$ such that $\sigma_n\in \mathbb{Z}^{k_n}$ and:
     $$X\subseteq\{x:\exists ^\infty _n \;\; \sigma_n\subseteq x\}.$$
 \end{proposition}


As it turns out, the characterization of strong measure zero sets provided in \ref{xdxdxd} does not hold in the Baire space, which we will demonstrate in Chapter 4. This motivates the following definition.

\begin{df}
 Set $X\in \mathcal{SMZ}^+$  if and only if for every interval partition $\bar{I}\in \mathbb{IP}$ there exists $z\in\mathbb{Z}^\omega$ such that:
 $$\forall x\in X\;\; \exists^\infty n\;\; x\upharpoonright I_n=z\upharpoonright I_n.$$
\end{df} 

\begin{proposition}
    $\mathcal{SMZ}^+$ forms a  $\sigma$-ideal in Baire space.
\end{proposition}

\begin{proof}
    Take $(X_l: l<\omega)$ where each $X_l \in \mathcal{SMZ}^+.$
    Take any interval partition $\bar{I}.$ We will construct a bigger partition $\bar{J}.$ Let:
    $$ J_n=I_{\frac{n\cdot(n-1)}{2}+n}\cup \cdots \cup I_{\frac{n\cdot(n-1)}{2}+2n}.$$ 
    
    Since every $X_l$ is in $\mathcal{SMZ}^+$ there exists $z_l$ for every $X_l$ such that: $$\forall x\in X_l \;\; \exists^\infty n  \;\; x\upharpoonright J_n= z_l\upharpoonright J_n.$$ We want to construct $z$ such that for every $l$, for all $x\in X_l $  there exists infinitely many $n$  such that $z\upharpoonright J_n= x\upharpoonright J_n$.
    
    Let $z\upharpoonright I_0 =z_1\upharpoonright I_0$.
    Next, if $k=\frac{n(n-1)}{2}+n\) for some \(n\) and $0<b<k+1$ define 
$z\upharpoonright I_k=z_1\upharpoonright I_k$ and  
  $z\upharpoonright I_{k+b}=z_{b+1}\upharpoonright I_{k+b}$.
\end{proof}



Of course we have $\mathcal{SMZ} \subseteq \mathcal{SMZ}^+$. In
Chapter $4$ we will show that under additional assumptions
the reverse inclusion does not hold. The following is a version of the Galvin-Mycielski-Solovay theorem
for the Baire space in terms of the ideals introduced above.

\begin{thm}
$\mathcal{M}_-^*=\mathcal{SMZ}^+$
\end{thm}

\begin{proof}
   To show $\mathcal{M}^*_-\subseteq\mathcal{SMZ}^+$ assume $X+H\neq \mathbb{Z}^\omega $ for any $H\in \mathcal{M_-}$. Take an interval partition $\bar{I}\in \mathbb{IP}$ and take $H\subseteq M(y,\bar{I})$, by translating $H$ we may assume that $y$ is constant with value $0$ on every coordinate. Since $X+H\neq \mathbb{Z}^\omega$ there exists $z\notin X+H\subseteq\bigcup_{x\in X} M(x,\bar{I}).$ So for every $x\in X$ there exists infinitely many $n $ such that $z\upharpoonright I_n = x\upharpoonright I_n$. So we get
    $X \in\mathcal{SMZ}^+.$

    To show $\mathcal{SMZ}^+\subseteq\mathcal{M}_-^*$
 take any $X\in \mathcal{SMZ}^+$ and any $H\in \mathcal{M}_-$, where $H\subseteq M(y,\bar{I})$ for some $y\in \mathbb{Z}^\omega$ and $\bar{I}\in \mathbb{IP}.$ Since $X\in \mathcal{SMZ}^+$ we have $X\subseteq\{x: \exists^{\infty} n \;\; x\upharpoonright I_n =z\upharpoonright I_n  \}$. We have $X+H\subseteq \bigcup_{x\in X} M(y+x,\bar{I})$. We have to show that there exists $a\notin X+H$. Let $a=y+z$.
Assume that $y+z\in X+H$, then for almost all $n$ and some $x\in X$ we have
$(y+x) \upharpoonright I_n \neq (y+z)\upharpoonright I_n$ , so $x\upharpoonright I_n\neq z\upharpoonright I_n$. 
We get a contradiction, because $X\in \mathcal{SMZ}^+$, so for infinitely many $n$ we have $x\upharpoonright I_n =z \upharpoonright I_n$.
\end{proof}

The next ideal we consider is the eventually different ideal, which was studied  in \cite{KHOMSKII}, where a tree dichotomy for this ideal was established.

\begin{df}
    Let $\mathcal{ED}$ be $\sigma$-ideal $\sigma$-generated by the sets $E_f$ where $f\in\mathbb{Z}^{\omega}$ and $$E_f=\{x\in\mathbb{Z}^{\omega}: \forall^{\infty}_n \;\; x(n)\neq f(n)\}.$$
\end{df}
When we write $E_n$ we mean $E_f$, where $f$ is constant with the value $n$.
\begin{proposition}\label{kkkkkkk}
    The ideal $\mathcal{ED}$ is properly contained in the ideal $\mathcal{M}_{-}$.
\end{proposition}
\begin{proof}
    Take any set $E_f$. Then  for any partition $\bar{I}$ we get  $E_f\subseteq M(f, \bar{I})\in \mathcal{M}_-.$

    Now we will show that the inclusion is proper. Let $X=M(0,\bar{I})$ where $\bar{I}$ is a partition into intervals such that $|I_n|=n+2$, say $I_n=\{i_0^n,_{\cdots}, i_{n+1}^n\}$. Assume there exists $(f_n)_{n<\omega}\subseteq \mathbb{Z}^\omega$ such that  $X\subseteq\bigcup_n E_{f_n}.$

    We will construct $x\in X $ such that $x\notin \bigcup_n E_{f_n}.$ Let:
    \begin{enumerate}
        \item $x(i_j^n)=f_j(i_j^n)$ for $j\leq n$,
        \item $x(i_{n+1}^n)=1$. 
    \end{enumerate}
    Of course we have $x\in X$ because of $(2)$ and $x\notin \bigcup_n E_{f_n}$ because of $(1).$
\end{proof}


In \cite{hruvsak2012cardinal}, Zindulka and Hru{\v{s}}{\'a}k extended the notion of porous sets from real line to the Cantor space.

\begin{df}
We say that a set $X\subseteq \mathbb{Z}^{\omega}$ is porous $(X\in \mathcal{P})$ if there exist $k$ such that for every $\sigma \in \mathbb{Z}^{m}$ there exists $\tau \in \mathbb{Z}^{m+k}$, $\sigma \subseteq \tau$ and $[\tau]\cap X=\emptyset.$   
  \end{df}
\begin{proposition}
    The ideal $\mathcal{M}_{-}$ is not contained in the ideal $\sigma\mathcal{P}$.
\end{proposition}
\begin{proof} 
    We will show that the set $M=\{x\in\Baire:\forall n\in\omega$ $x|_{I_{n}}\neq0|_{I_{n}}\}\in\mathcal{M}_{-}$, where $(I_{n})_{n\in\omega}$ is an interval partition made of intervals of increasing length, is not in $\notin\sigma\mathcal{P}$. Assume that $M\subseteq \bigcup_{n}P_{n}$ where every $P_{n}$ is $k_{n}$-porous. On the one hand, by Baire category theorem there is $\sigma\in\omega^{<\omega}$ and $n\in\omega$ such that $M\cap[\sigma]\subseteq P_{n}$. On the other, it is not difficult to construct $y\in (M\cap[\sigma])\setminus P_{n}$.
\end{proof}
\begin{proposition}
    The ideal $\mathcal{ED}$ is not contained in the ideal $\mathcal{P}$(we need $\sigma\mathcal{P}$).
\end{proposition}
\begin{proof}
    %Take $E_0$. There exists $\{A_m: \alpha<\omega\}$ such that every $A_m\subseteq E_0.$ For every $x\in A_m$ we want $\forall n>m\;\; x(n)\neq 0$ and bellow $m$ let  $x $ be any natural number. Let $\bigcup A_m =X$

    Assume $E_0$ is $k$-porous. Take  any $
    \sigma\in \mathbb{Z}^n$. Take any $\tau\in\mathbb{Z}^{n+k}$ such that $\sigma\subseteq \tau$. Take $x\in\mathbb{Z}^{\omega}$ such that for $s\leq n+k+1$ we have $x(s)=\tau (s)$. And for $s>n+k+1$ let $x(s)=1$. Of course $x\in E_0$ and $x\in [\tau]$, so $E_0\notin\mathcal{P}.$    
\end{proof}



\begin{df}
    Let $\mathcal{IE}$ be $\sigma$-ideal $\sigma$-generated by $I_g$ where $g\in \mathbb{Z}^\omega$ and $$I_g=\{x\in \mathbb{Z}^\omega:\exists^\infty n \;\; x(n)=g(n)\}.$$
\end{df}
 We will be also interested in the following ideal that was implicitly  used by Bartoszyński and Judach in \cite{BBB} to characterize $\add(\mathcal{M})$ and $\cof(\mathcal{M}).$ 
\begin{df}
    Let $\mathcal{H}$ be $\sigma$-ideal generated by $H({f,\bar{I}})$ where $f\in\mathbb{Z}^{\omega}$, $\bar{I}\in \mathbb{IP} $ and $$H({f,\bar{I}})=\{x\in\mathbb{Z}^{\omega}: \forall^{\infty}n \exists m\in I_n \;\; x(m)= f(m)\}.$$
\end{df}

Note that  for every $ (\bar{I}^n)_{n<\omega}\in \mathbb{IP}$ and every $(f_n)_{n<\omega}\in \mathbb{Z}^\omega$ there is $\bar{J}\in \mathbb{IP}$ and $g\in \mathbb{Z}^\omega$ such that $\bigcup_{n} H({f_n,\bar{I}^n})\subseteq H({g, \bar{J}})$.




\begin{proposition}
    The ideal $\mathcal{H}$ is properly contained $\mathcal{M}_-$.
\end{proposition}

\begin{proof}
    For any $H({f, \bar{I}})\in \mathcal{H}$ we have $H({f,\bar{I}})\subseteq M(f+1,\bar{I}).$

Now we will show that this inclusion is proper. 
Let $X=M(0,\bar{I})$ where $\bar{I}$ is a partition into singletons. Assume there exists $\bar{J}\in\mathbb{IP},f\in \mathbb{Z}^\omega$ such that $M(0,\bar{I})\subseteq H({f,\bar{J}})$. We will construct $x\in \mathbb{Z}^\omega$ as follows:
\begin{itemize}
    \item [--]  If $f(n)\neq 1$, let $x(n)=f(n)-1$,
    \item [--]  if $f(n)=1$ let $x(n)=2$.

\end{itemize}

Of course $x\in M(0,\bar{I})$ and $x\notin H({f,\bar{J}}).$
\end{proof}


\begin{proposition}
    The ideal $\mathcal{H}$ is properly contained in the ideal $\mathcal{IE}$.
\end{proposition}

\begin{proof}
    Note that for any $H({f,\bar{I}})\in \mathcal{H}$ we have $H({f, \bar{I}})\subseteq I_f$.

Now we will show that the inclusion is proper.
Take any set $I_f\in \mathcal{IE}.$ Assume that $I_f\subseteq H({f, \bar{I}})$ for some interval partition $\bar{I}.$ But there exists $x\in I_f$ such that for every $k$ and every $m\in I_{2k}$ we have $x(m)\neq f(m).$
\end{proof}

\begin{df}
 Set $X\in \mathcal{G}$  if and only if for every interval partition $\bar{I}\in \mathbb{IP}$ there exists $z\in\mathbb{Z}^\omega$ such that:
 $$\forall x\in X\;\; \exists^\infty n\;\; \forall m\in I_n \;\; x(m)\neq z(m).$$
\end{df} 

\begin{proposition}
    $\mathcal{G}$ forms a $\sigma$-ideal in the Baire space.
\end{proposition}

\begin{proof}
    Assume that $\{X_l: l<\omega\}\subseteq\mathcal{G}$ and let $\bar{I}$ be an interval partition. Let $\bar{J}=(J_{n})_{n\in\omega}$ be such interval partition that:
   $$J_n=I_{\frac{n\cdot(n-1)}{2}+n}\cup \cdots  \cup  I_{\frac{n\cdot(n-1)}{2}+2n}.$$
    Since every $X_l$ is in $\mathcal{G}$ there exists $z_l$ for every $X_l$ such that: \[\forall x\in X_l \;\; \exists^\infty n\; \forall m\in J_n\; x(m)\neq z_l(m).\] We will construct $z$ such that for every $l$, for every  $x\in X_l$ there exists infinitely many $n$ such that for every $m\in J_n \;\; z(m)\neq x(m)$. 
    
    Let $z\upharpoonright I_0 =z_1\upharpoonright I_0$.
    Next, if $k=\frac{n(n-1)}{2}+n\) for some \(n\) and $0<b<k+1$ define 
$z\upharpoonright I_k=z_1\upharpoonright I_k$ and  
  $z\upharpoonright I_{k+b}=z_{b+1}\upharpoonright I_{k+b}$.
\end{proof}

\begin{proposition}
    $\mathcal{ED}\subseteq\mathcal{G}$ (properly ?).
\end{proposition}
\begin{proof}
    Take any $E_f\in \mathcal{ED}$. To show that $E_f \in \mathcal{G}$ take any partition $\bar{I}$. Take $f$. Of course for every $x\in E_f$, there exist infinitely many $n$ such that for every $m\in I_n$ we have $f(m)\neq x(m),$ because for every $x\in E_f$ we have $x\neq^*f.$    
\end{proof}




We will next study the ideal of uniformly meager set introduced in \cite{umeager}(na pewno?).
\begin{df}
    Set $X\subseteq\mathbb{Z}^\omega$ is uniformly nowhere dense if for every $k\in\omega$ there exists $l\in \omega$ such that for every $\tau\in \mathbb{Z}^k$ there exists $\sigma\in \mathbb{Z}^{k+l}$ such that $\tau\subseteq\sigma$ and $[\sigma]\cap X=\emptyset$.     Set $X\subseteq\mathbb{Z}^\omega$ $(X\in \mathcal{UM})$ is uniformly meager if it is a countable union of uniformly nowhere dense sets.
\end{df}
Clearly, we have $\mathcal{P}\subseteq \mathcal{UM}\subseteq\mathcal{M}$. The ideal $\mathcal{UM}$ can analogously be defined in any Polish group and in \cite{umeager} authors showed that a Polish group is locally compact if and only if the ideal of meager set and the ideal of uniformly meager sets coincide.\\
Now we will introduce a characterization of uniformly meager sets in the spirit of REF CHOPPED REALS that we will frequently use later on.


The inclusions discussed above are illustrated in the diagram below. All inclusions are proper, with proof of $\mathcal{ED}\neq \mathcal{G}$ provided in chapter $4$ under assumption of $\add(\mathcal{H})=\mathfrak{c}.$

\begin{center}
\begin{tikzpicture}[node distance=1.5cm, auto]
    % Definicja punktów (węzłów)
    \node (M) at (0, 4.5) {$\mathcal{M}$};
    \node (MM) at (0, 3) {$\mathcal{UM}$};
    \node (Mminus) at (0, 1.5) {$\mathcal{M}_-$};
    \node (IE) at (-2, 1.5) {$\mathcal{IE}$};
    \node (G) at (3, 1.5) {$\mathcal{G}$};
    \node (P) at (1.5, 1.5) 
    {$\sigma$-$\mathcal{P}$};
    \node (H) at (-1, 0) {$\mathcal{H}$};
    \node (ED) at (1.5, 0) {$\mathcal{ED}$};

    % Rysowanie strzałek
    \draw[->] (H) -- (IE);
    \draw[->] (H) -- (Mminus);
        \draw[->] (ED) -- (P);
            \draw[->] (P) -- (MM);
    \draw[->] (ED) -- (Mminus);
    \draw[->] (ED) -- (G);
    \draw[->] (Mminus) -- (MM);
    \draw[->] (MM) -- (M);
\end{tikzpicture}
\end{center}



If we consider the same definitions in the Cantor space, some of the definitions collapse.


\begin{proposition}
    

    In Cantor space $\mathcal{H}(2^\omega)=\mathcal{M}_-(2^\omega)=\mathcal{UM}(2^\omega)=\mathcal{M}(2^\omega)$.
    \end{proposition}

\begin{proof}
    By \ref{XD} $\mathcal{M}_-(2^\omega)=\mathcal{UM}(2^\omega)$
    We only need to show that in Cantor space $\mathcal{M}_-(2^\omega) \subseteq\mathcal{H}(2^\omega)$. Take any $x\in\mathcal{M_-}(2^\omega)$. We know that $X\subseteq M(x,\bar{I})$ for some $x\in 2^\omega$ and $\bar{I}\in \mathbb{IP}.$ We have $X\subseteq H({x+1, \bar{I}})$.
\end{proof}

\begin{proposition}
    

    In Cantor space $\mathcal{G}(2^\omega)=\mathcal{SMZ}^+(2^\omega)=\mathcal{SMZ}(2^\omega)$.
\end{proposition}

\begin{proof}
    By \ref{xdxdxd} we know that $\mathcal{SMZ}(2^\omega)=\mathcal{SMZ}^+(2^\omega)$.
        We only need to show that in Cantor space $\mathcal{G}(2^\omega) \subseteq\mathcal{SMZ}^+(2^\omega)$. Take any $X\in\mathcal{G}(2^\omega)$ and any partition $\bar{I}\in \mathbb{IP}$. We will find $z\in 2^\omega$ such that for every $x\in X $ there exist infinitely many $n$ such that $ x\upharpoonright I_n=z\upharpoonright I_n$.
        Since $X\in \mathcal{G}(2^\omega)$ we know that there exists $y\in2^\omega$ such that for every $ x\in X$ there exists infinitely many $n$  such that for every $  m\in I_n $ we have  $ x(m)\neq y(m)$.
        Let $z=y+1.$
\end{proof}



$\mathcal{ED}$ na Cantorze to Countable

Na Cantorze $\mathcal{M}\subseteq \mathcal{IE}$, trywialny ideał

$\sigma$-$\mathcal{P}$ dorzucić na diagram i gdzie są na Cantorze

==> other_proofs.tex <==
\begin{proof}
    
    \begin{itemize}
        \item $add(\mathcal{H})\leqslant add (\mathcal{M})$
        \end{itemize}
        First we have to prove that $add(\mathcal{H})\leq cov(\mathcal{M})$. Take $\{x_\alpha : \alpha<cov(\mathcal{M})\}=F$. Take $H({x_\alpha, \bar{I}})$. Assume that there exists $H({y,\bar{J}})$ such that $\bigcup_{\alpha < cov(\mathcal{M})} H({x_\alpha,\bar{I}}) \subseteq H({y,\bar{J}})$. But since $F$ is of size $cov(\mathcal{M})$ we can find $x_\alpha $ such that for almost all $n$ we have $x_\alpha (n)\neq y(n).$ So we get $H({x_\alpha, \bar{I}}) \nsubseteq H({y, \bar{J}})$

        Next we need to show that $add(\mathcal{H})\leq \mathfrak{b}$. Take $\{H({x_\alpha, \bar{I^\alpha}}):\alpha< \mathfrak{b}\}$ such that $I^\alpha$ is an unbounded family. Assume that there exists $H({y,\bar{J}} $ such that $\bigcup H({x_\alpha, \bar{I^\alpha}}) \subseteq H({y,\bar{J}})$. So for every $\alpha $ we have $H({x_\alpha, \bar{I^\alpha}}) \subseteq H({y,\bar{J}}).$ So by Lemma \ref{sssss} we get for every $ \alpha \quad I^\alpha \sqsubseteq ^* J.$ we get a contradiction because $I^\alpha$ was unbounded family.
 \begin{itemize}

        \item $add(\mathcal{H})\geqslant add (\mathcal{M})$
            \end{itemize}
        Assume we have $add(\mathcal{H})<\kappa<\add(\mathcal{M})$. Take $\{H^\alpha: \alpha<\kappa\}$, where $H^\alpha=H({x_\alpha , \bar{I^\alpha}})$.

        We will show that $\bigcup_{\alpha<\kappa} H^\alpha\subseteq \mathcal{H}$

        For every $\alpha$, we will construct $z_\alpha\in\mathbb{Z}^\omega$ such that $z_\alpha(n)=\text{"} x_\alpha \upharpoonright I^\alpha_n \text{"}$.

        Since $\kappa<\add(\mathcal{M})$ we can find $c$ such that for all $\alpha$ there exist infinitely many $n$ such that $z_\alpha(n)=c(n)$

        Now we want to construct $d$ in such a way that if $z_\alpha(n)=c(n)$ let $d\upharpoonright I^\alpha_n=x_\alpha\upharpoonright I^\alpha_n.$ If $z_\alpha(n)\neq c(n)$ let $d\upharpoonright I^\alpha_n=0$.

        Next let $I^\alpha\sqsubseteq^* J^\alpha$ such that for all $n$ there exists $k$ such that $I^\alpha_k \subseteq J^\alpha_n$ and $x_\alpha \upharpoonright I^\alpha_k =d \upharpoonright I_k^\alpha.$ 

        Now because $\kappa<add(\mathcal{M)}$ take $R\in \mathbb{IP}$ such that for all $\alpha $ $J^\alpha\sqsubseteq^*R$.

        Of course $\bigcup_{\alpha<\kappa} H({x_\alpha, I^\alpha}) \subseteq H({d,R}).$

        
        

    
\end{proof}


\begin{thm}
    $\cof(\mathcal{H})=\cof(\mathcal{M})$
\end{thm}

\begin{proof}
We will again use characterization $\cof(\mathcal{M})=\min\{\mathfrak{d},\non(\mathcal{M})\}$.

First, we will show that $cof(\mathcal{H})\geqslant \mathfrak{d}$
Let $F\{H_{I^\alpha,x_\alpha}: \alpha< \cof(\mathcal{M})\}$ be a basis of $\mathcal{H.}$ Take any $y\in \omega^\omega
$ and any $J\in \mathbb{IP}.$ There exists $\alpha$ such that $H_{J,y}\subseteq H_{I^\alpha,x_\alpha}$. So by \ref{sssss} we get $J\sqsubseteq^* I^\alpha$. And we get that   family $\{I^\alpha:\alpha<cof(\mathcal{M})\}$ is a dominating family.

    Next we will show that $\cof(\mathcal{H})\geqslant \non (\mathcal{M})$.  

 Let $\{H(x_\alpha, I^\alpha): \alpha< \cof(\mathcal{M})\}$ be a basis of $\mathcal{H}$. We will show that set $F=\{x_\alpha: \alpha<\cof(\mathcal{H})\} $ is of size $\non(\mathcal{M}).$ Take any $y\in \omega^\omega$. We know that for any interval partition $\bar{I}$ we have $H(y, \bar{I})\subseteq H(x_\alpha, I^\alpha).$ So for infinitely many $n$ we have $x_\alpha(n)=y(n)$ so from \ref{xd} family $F$ is of size $\non(\mathcal{M}).$




     Now we will prove that $\cof(\mathcal{H})\leqslant \cof (\mathcal{M})$

        Let $\langle\bar{I}^\alpha: \alpha<\mathfrak{d}\rangle$ be a dominating family in $\mathbb{IP}$ and for $\alpha<\mathfrak{d}$ let $\langle f^\alpha_\gamma: \gamma<\non(\mathcal{M})\rangle$ be such that for every $f\in \omega^\omega$ there exists $\gamma$ such that for infinitely many $n$ we have $f\upharpoonright I_n^\alpha= f_\gamma^\alpha\upharpoonright I_n^\alpha$. Let $H^{\alpha, \beta}_\gamma= H(\bar{I}^\beta, f^\alpha_\gamma).$ 
        
        \begin{claim}
            $\langle H^{\alpha, \beta}_\gamma: \alpha, \beta<\mathfrak{d}, \gamma<\non(\mathcal{M})\rangle$ is a basis of $\mathcal{H}$.
        \end{claim}
        Take any $H(x, \bar{J})$. Of course we can find $\alpha$ such that $H(x,\bar{J})\subseteq H(x, \bar{I}^\alpha)$. There exists $f^\alpha_\gamma$ such that for infinitely many $n$ we have $x\upharpoonright I_n^\alpha=f_\gamma^\alpha\upharpoonright I_n^\alpha$.  Take interval partition $\bar{R}$ such that for almost all $n$ there exists $k$ such that $I^\alpha_k\subseteq R_n$ and $x\upharpoonright I_k^\alpha =f^\alpha_\gamma\upharpoonright I_k^\alpha.$ Take $I^\beta$ such that $R\sqsubseteq^* I^\beta$. Of course $H(x,\bar{J})\subseteq H(f^\alpha_\gamma
        , I^\beta)$
\end{proof}



\begin{thm}
    For any analytic $A\subseteq\omega^{\omega}$ either $A\in \mathcal{H}$ or there is a tree $T \in \mathbb{T}_{\mathcal{H}}$ such that $[T]\subseteq A$. In particular, the assignment 
    \begin{center}
        $\mathbb{T}_{\mathcal{H}}\ni T\longmapsto [T]\in Bor /{\mathcal{H}}$
    \end{center} is a dense embedding and the forcing notions $(\mathbb{T}_{\mathcal{H}}, \subseteq)$ and $(Bor /{\mathcal{H}}, \subseteq)$ are forcing equivalent.
\end{thm}
    \begin{proof}
         Let $T$ be a tree on $\omega \times \omega$ such that $A=\pi[[T]]$ (here $\pi$ denote the projection on to the first coordinate). For any tree $S$ on $\omega \times \omega$ define the derivative:
  $$S'=\{(\sigma,\tau)\in S:(\exists M>|\sigma|) (\forall I\subseteq \omega\backslash M)(\forall \rho \in \omega^I)$$$$(\exists (\sigma',\tau')\in S\upharpoonright_{(\sigma,\tau)}) (\forall n\in I \;\;\sigma'(n) \neq\rho(n))\}.$$

Next, we will inductively define:
\begin{itemize}
    \item [--]  $T^{0}=T$,
    \item [--]$T^{\alpha+1}=\left(T^{\alpha}\right)^{\prime}$,
    \item  [--]$T^{\lambda}=\bigcap_{\alpha<\lambda} T^{\alpha}$ for limit ordinal $\lambda$.
\end{itemize}

Let $\alpha_0<\omega_1$ be the least such that $T^{\alpha_0}=T^{\alpha_0+1}$. Consider the following two cases:

Case $1)$  $T^{\alpha_0}=\emptyset$.

Note that $[\pi (T)]\subseteq \bigcup_{\beta < \alpha_0} [\pi [T^\beta \backslash T^{\beta +1}]].$ It will be enough to show that for every $\beta<\alpha_0$ we have $[\pi[T^\beta\setminus T^{\beta+1}]]\in \mathcal{ H}.$ Fix $\beta<\alpha_0$ and $(\sigma, \tau)\in T^\beta \backslash T^{\beta+1}.$ We will show that $[\pi [T^\beta\upharpoonright_{(\sigma, \tau)}]]\in \mathcal{H}$.

Since $(\sigma, \tau )\notin T^{\beta+1}$ we get:
$$\forall  M >|\sigma|=|\tau|\;\; \exists I\subseteq \omega\backslash M \;\; \exists \rho \in \omega^I \;\; \forall (\sigma',\tau')\in T^\beta \upharpoonright_{(\sigma, \tau)} $$$$ \exists m\in I \;\;\sigma'(m)= \rho(m) .\;\; \;\; (*)$$

 We will inductively build $x\in \omega^\omega$ and an interval partition $J=(J_{n})_{n\in\omega}$ such that $[\pi[T^\beta \upharpoonright_{(\sigma ,\tau )}]]\subseteq H_{J,x}.$ 

Assume that $J_n$ and $x\upharpoonright J_n$ has been constructed. By $(*)$ there is an interval $I_n\subseteq \omega \backslash \max(J_n)$ and $\rho_n \in \omega^{I_n}$ such that:
$$
\forall (\sigma',\tau') \in T^\beta \upharpoonright _{(\sigma,\tau)} \;\; \exists  m \in I_n \;\;\sigma'(m)=\rho_n(m) \;\;\;(**). 
%\;\; \;\; 
$$

Let  $J_{n+1}=[\max(J_n)+1, \max (I_n)]$ and  let $x\upharpoonright  J_{n+1}$ be such that $x\upharpoonright I_n =\rho_n$.\\
We claim that $[\pi [T^\beta \upharpoonright _{(\sigma, \tau)}]] \subseteq H_{J,x}$. 

Take any $y\in [\pi [T^\beta \upharpoonright _{(\sigma, \tau)}]]$. There exists $z\in\omega^{\omega}$ such that $(y,z)\in T^\beta \upharpoonright_{(\sigma,\tau)}$. So by $(**)$  for every $n$ there exists $m\in I_n$ such that  $y(m)= \rho_{n}(m)$. Since $I_n\subseteq J_n$ for every $n\in\omega$, we can find $m\in I_n$ such that  $y(m)= x(m)$ and it holds for almost all $n\in\omega$. It follows that  $y\in H_{J,x}$.

Case $2)$  $T^{\alpha_0}\neq \emptyset$.

We will show that $\pi [T^{\alpha_0}] \in \mathbb{T}_{\mathcal{H}} $.



Let $\sigma \in \pi [T^{\alpha_0}]$ and let $\tau$ be  such that $(\sigma, \tau) \in T^{\alpha_0}.$ As $T^{\alpha_{0}}=T^{\alpha_{0}+1}$ there is $M>|\sigma|=|\tau|$ such that for every interval $I\subseteq \omega \backslash M$ and for every $\rho\in\omega ^I$ we can find $(\sigma',\tau')\in T^{\alpha_0}\upharpoonright_{(\sigma,\tau)}$ and for every  $n\in I$ we have  $\sigma'(n)\neq\rho(n)$. 
\end{proof}



\begin{proposition}
    $\mathbb{T}_{\mathcal{M}_-}$ does not have $c.c.c.$
\end{proposition}
\begin{proof}
    For every $x\in 2^\omega$ we will create a tree $T_x\in\mathbb{T}_{\mathcal{M}_-}$ such that for $x\neq y$ we have $[T_x]\cap [T_y]=\emptyset$. Enumerate $\omega^{<\omega}$ as $\{\sigma_n:n<\omega\}$. For $x\in2^\omega$ inductively construct an increasing sequence $\{F_n^x:n<\omega\}$ well founded trees as follows: if $F_n^x$ has been done, then define 
    \begin{center}
        $F^x_{n+1}=\bigcup\{\tau^\frown n^\frown x(n+1):n<\omega $ and $\tau\in term(F_n^x)\}$
    \end{center}
    Define now $T_x=\bigcup_n F_n^x$. It is not difficult to see that $T_x\in\mathbb{T}_{\mathcal{M}_-}$ and for $x\neq y$ in $2^{\Cantor}$ we have that $[T_x]\cap [T_y]=\emptyset$.
\end{proof}
